MotionGS : Compact Gaussian Splatting SLAM by Motion Filter

With their high-fidelity scene representation capability, the attention of SLAM field is deeply attracted by the Neural Radiation Field (NeRF) and 3D Gaussian Splatting (3DGS). Recently, there has been a surge in NeRF-based SLAM, while 3DGS-based SLAM is sparse. A novel 3DGS-based SLAM approach with a fusion of deep visual feature, dual keyframe selection and 3DGS is presented in this paper. Compared with the existing methods, the proposed tracking is achieved by feature extraction and motion filter on each frame. The joint optimization of poses and 3D Gaussians runs through the entire mapping process. Additionally, the coarse-to-fine pose estimation and compact Gaussian scene representation are implemented by dual keyframe selection and novel loss functions. Experimental results demonstrate that the proposed algorithm not only outperforms the existing methods in tracking and mapping, but also has less memory usage.

==> cvpr_header.tex <==
\ifreview \usepackage[review]{cvpr} \fi
\ifarxiv \usepackage[pagenumbers]{cvpr} \fi
\ifrebuttal \usepackage[rebuttal]{cvpr} \fi
\ifcamera \usepackage{cvpr} \fi

\input{_macros}  % Add packages to _macros.tex

%% For cross-referencing labels between documents
\usepackage{xr-hyper}

\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}

\makeatother
\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%

\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}

\ifarxiv \crefname{appendix}{App.}{Apps.}
\else \crefname{appendix}{Suppl.}{Suppls.} \fi

\frenchspacing


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/compare_render.tex <==
\begin{table}[t]
\centering
\resizebox{0.83\textwidth}{!}{%

\begin{tabular}{c@{\hspace{0.05cm}}c@{\hspace{0.05cm}}c}
  MonoGS  & SplaTAM &  Ours  \\
\includegraphics[width=0.3\textwidth]{figs/pictures/desk-monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/desk-splatam.png}  &
\includegraphics[width=0.3\textwidth]{figs/pictures/desk-my.png} 
 
\\
\includegraphics[width=0.3\textwidth]{figs/pictures/xyz_monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/xyz_splatam.png}  &
\includegraphics[width=0.3\textwidth]{figs/pictures/xyz-my.png} 
 
\\
\includegraphics[width=0.3\textwidth]{figs/pictures/long-monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/long-splatam.png}  &
\includegraphics[width=0.3\textwidth]{figs/pictures/long-my.png} 
 
\\
\end{tabular}

}
\caption{
\textbf{Render Performence in TUM}. The datasets from top to bottom are desk, xyz, long\_office.
}

\vspace{-0.05in}
\label{tab:render_tum}
\end{table}

==> tables/compare_render_replica.tex <==
\begin{table}[htbp]
\centering
\resizebox{0.6\textwidth}{!}{

\begin{tabular}{ccc}
  MonoGS  & SplaTAM &  Ours  \\
\includegraphics[width=0.3\textwidth]{figs/pictures/room0_monogs.png} & \!
\includegraphics[width=0.3\textwidth]{figs/pictures/room0_splatam.png}  & \!
\includegraphics[width=0.3\textwidth]{figs/pictures/room0_my.png} 
 
\\
\includegraphics[width=0.3\textwidth]{figs/pictures/room1_monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/room1_splatam.png}  &
\includegraphics[width=0.3\textwidth]{figs/pictures/room1_my.png} 
 
\\
\includegraphics[width=0.3\textwidth]{figs/pictures/room2_monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/room2_splatam.png}  &
\includegraphics[width=0.3\textwidth]{figs/pictures/room2_my.png} 
 
\\
\includegraphics[width=0.3\textwidth]{figs/pictures/office0-monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office0_splatam.png}  &
\includegraphics[width=0.3\textwidth]{figs/pictures/office0-my.png} 
 
\\
\includegraphics[width=0.3\textwidth]{figs/pictures/office1-monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office1_splatam.png}  &
\includegraphics[width=0.3\textwidth]{figs/pictures/office1_my.png} 
 
\\
\includegraphics[width=0.3\textwidth]{figs/pictures/office2-monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office2_splatam.png}  &
\includegraphics[width=0.3\textwidth]{figs/pictures/office2-my.png} 
 
\\
\includegraphics[width=0.3\textwidth]{figs/pictures/office3-monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office3_splatam.png}  &
\includegraphics[width=0.3\textwidth]{figs/pictures/office3_my.png} 
 
\\
\includegraphics[width=0.3\textwidth]{figs/pictures/office4-monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office4_splatam.png}  &
\includegraphics[width=0.3\textwidth]{figs/pictures/office4-my.png} 
 
\\
\end{tabular}

}
\caption{
\textbf{Render Performence in Replica}. The datasets from top to bottom are r0, r1, r2, o0, o1, o2, o3. Our rendering effect with better detail representation ability has been demonstrated by the  clocks, flower pots, murals, books and so on.  
}

\vspace{-0.05in}
\label{tab:render_replica}
\end{table}

==> tables/contribution.tex <==
\begin{table}[t]
\centering
% \resizebox{\columnwidth}{!}{%


\caption{
Caption goes here
}
\vspace{-0.05in}
\label{tab:template}
\end{table}


==> tables/renderinreplica.tex <==
\renewcommand{\arraystretch}{0.5}
\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{

\begin{tabular}{c@{\hspace{0.05cm}}c@{\hspace{0.05cm}}c@{\hspace{0.05cm}}c@{\hspace{0.05cm}}c@{\hspace{0.05cm}}c@{\hspace{0.05cm}}c@{\hspace{0.05cm}}c@{\hspace{0.05cm}}c}
~ & \textbf{Room0}  & \textbf{Room1} & \textbf{Room2} & \textbf{Office0} & \textbf{Office1} & \textbf{Office2} & \textbf{Office3} & \textbf{Office4}  \\
\rotatebox{90}{\begin{tabular}{@{\hspace{0.3cm}}c@{}}\textbf{MonoGS}\end{tabular}}  & \includegraphics[width=0.3\textwidth]{figs/pictures/room0_monogs.png} & \includegraphics[width=0.3\textwidth]{figs/pictures/room1_monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/room2_monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office0-monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office1-monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office2-monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office3-monogs.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office4-monogs.png}

\\
\rotatebox{90}{\begin{tabular}{@{\hspace{0.275cm}}c@{}}\textbf{SplaTAM}\end{tabular}}  & \includegraphics[width=0.3\textwidth]{figs/pictures/room0_splatam.png} & \includegraphics[width=0.3\textwidth]{figs/pictures/room1_splatam.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/room2_splatam.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office0_splatam.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office1_splatam.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office2_splatam.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office3_splatam.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office4_splatam.png}
\\

\rotatebox{90}{\begin{tabular}{@{\hspace{0.73cm}}c@{}}\textcolor{red}{\textbf{Ours}}\end{tabular}} & \includegraphics[width=0.3\textwidth]{figs/pictures/room0_my.png} & \includegraphics[width=0.3\textwidth]{figs/pictures/room1_my.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/room2_my.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office0-my.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office1_my.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office2-my.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office3_my.png} &
\includegraphics[width=0.3\textwidth]{figs/pictures/office4-my.png}
\end{tabular}

}
\caption{
\textbf{Render Performence in Replica}. Our rendering effect with better detail representation ability has been demonstrated by the  clocks, flower pots, murals, books and so on.  
}
\vspace{-0.05in}
\label{tab:render_replica2}
\end{table}
